Dynamical Masses and Mass-to-light Ratios of Resolved Massive Star Clusters. I. NGC 419 and NGC 1846

As an introduction of a kinematic survey of Magellanic Cloud (MC) star clusters, we report on the dynamical masses and mass-to-light ($M/L$) ratios of NGC 419 (SMC) and NGC 1846 (LMC). We have obtained more than one hundred high-resolution stellar spectra in and around each cluster using the multi-object spectrograph M2FS on the $Magellan$/Clay Telescope. Line-of-sight velocities and positions of the stars observed in each cluster were used as input to an expectation-maximization algorithm used to estimate cluster membership probabilities, resulting in samples of 46 and 52 likely members ($P_{M}\geq 50$%) in NGC 419 and NGC 1846, respectively. This process employed single-mass King models constrained by the structural parameters of the clusters and provided self-consistent dynamical mass estimates for both clusters. Our best-fit results show that NGC 419 has a projected central velocity dispersion of $2.44^{+0.37}_{-0.21}\ {\rm km\,s^{-1}}$, corresponding to a total mass of $7.6^{+2.5}_{-1.3}\times10^4\ {\rm M}_{\odot}$ and $V$-band $M/L$ ratio of $0.22^{+0.08}_{-0.05}$ in solar units. For NGC 1846, the corresponding results are $2.04^{+0.28}_{-0.24}\ {\rm km\,s^{-1}}$, $5.4^{+1.5}_{-1.4}\times10^4\ {\rm M}_{\odot}$ and $0.32^{+0.11}_{-0.11}$. The mean metallicities of NGC 419 and NGC 1846 are found to be $\rm [Fe/H]=-0.84\pm0.19$ and $-0.70\pm0.08$, respectively, based on the spectra of likely cluster members. We find marginal statistical evidence of rotation in both clusters, though in neither cluster does rotation alter our mass estimates significantly. We critically compare our findings with those of previous kinematic studies of these two clusters in order to evaluate the consistency of our observational results and analytic tools.

==> tab/t4_full.tex <==
\begin{table*}
\caption{M2FS Sample of NGC 419.}
\label{tab:sample_n419}
\begin{threeparttable}
\begin{tabular}{cccccccc}
\hline
{ID} & {$\alpha_{2000}$} & {$\delta_{2000}$} & {$V$} & {$V-I$} & {$v_{\rm los}$} & {$P_{M_i}$} & {Sel. $^{\rm a}$}\\ 
{ } & {(h:m:s)} & {($^{\circ}$:$\arcmin$:$\arcsec$)} & {(mag)} & {(mag)} & {(km\,s$^{-1}$)} & { } & { } \\
\hline
N419-1-b001 & 01:08:44.19 & -73:00:40.0 & $16.887\pm0.047$ & $1.497\pm0.055$ & $188.41\pm0.20$ & $0.00$ & M \\
N419-1-b002 & 01:08:46.07 & -72:56:35.2 & $17.942\pm0.030$ & $1.024\pm0.056$ & $192.79\pm0.42$ & $0.00$ & M \\
N419-1-b003 & 01:08:45.46 & -72:55:15.4 & $17.982\pm0.030$ & $1.138\pm0.043$ & $153.30\pm0.39$ & $0.00$ & M \\
N419-1-b004 & 01:08:43.26 & -72:53:32.0 & $18.014\pm0.008$ & $0.855\pm0.010$ & $193.60\pm0.61$ & $0.06$ & H \\
N419-1-b005 & 01:08:42.25 & -72:53:12.3 & $18.769\pm0.010$ & $1.019\pm0.013$ & $144.09\pm1.05$ & $0.00$ & H \\
N419-1-b006 & 01:08:36.93 & -72:53:08.6 & $18.072\pm0.007$ & $1.153\pm0.009$ & $188.79\pm0.36$ & $0.95$ & H \\
N419-1-b007 & 01:08:45.63 & -72:53:00.6 & $16.447\pm0.005$ & $1.721\pm0.005$ & $188.41\pm0.19$ & $0.89$ & H \\
N419-1-b008 & 01:08:42.71 & -72:52:36.2 & $18.742\pm0.012$ & $1.156\pm0.014$ & $163.46\pm0.75$ & $0.00$ & H \\
N419-1-b009 & 01:08:46.44 & -72:59:58.8 & $18.888\pm0.090$ & $0.809\pm0.139$ & $147.99\pm2.12$ & $0.00$ & M \\
N419-1-b010 & 01:08:53.00 & -72:59:08.5 & $18.126\pm0.074$ & $1.334\pm0.113$ & $191.09\pm0.88$ & $0.00$ & M \\
N419-1-b011 & 01:09:36.98 & -72:58:13.9 & $18.951\pm0.040$ & $0.873\pm0.058$ & $131.76\pm0.77$ & $0.00$ & M \\
N419-1-b012 & 01:09:10.13 & -72:57:30.3 & $16.764\pm0.108$ & $1.687\pm0.130$ & $171.52\pm0.27$ & $0.00$ & M \\
N419-1-b013 & 01:09:25.91 & -72:55:17.1 & $18.384\pm0.031$ & $1.030\pm0.054$ & $160.83\pm0.71$ & $0.00$ & M \\
N419-1-b015 & 01:08:52.25 & -72:53:57.3 & $18.896\pm0.088$ & $1.096\pm0.096$ & $134.17\pm0.93$ & $0.00$ & M \\
N419-1-b017 & 01:09:11.83 & -72:48:22.3 & $17.250\pm0.029$ & $1.316\pm0.039$ & $180.94\pm0.47$ & $0.00$ & M \\
N419-1-b018 & 01:09:03.45 & -72:50:13.0 & $18.416\pm0.119$ & $0.778\pm0.126$ & $204.86\pm1.45$ & $0.00$ & M \\
N419-1-b019 & 01:08:45.59 & -72:50:52.7 & $18.672\pm0.009$ & $1.140\pm0.011$ & $190.08\pm0.53$ & $0.94$ & H \\
N419-1-b020 & 01:08:40.43 & -72:51:00.7 & $17.596\pm0.007$ & $1.011\pm0.009$ & $187.88\pm0.33$ & $0.70$ & H \\
N419-1-b021 & 01:09:49.97 & -72:51:21.8 & $17.449\pm0.032$ & $1.404\pm0.043$ & $151.76\pm0.37$ & $0.00$ & M \\
N419-1-b022 & 01:08:42.54 & -72:51:27.5 & $18.392\pm0.009$ & $0.871\pm0.011$ & $146.39\pm0.58$ & $0.00$ & H \\
N419-1-b024 & 01:08:38.89 & -72:52:05.9 & $18.954\pm0.012$ & $1.048\pm0.014$ & $184.06\pm0.90$ & $0.01$ & H \\
N419-1-b025 & 01:08:33.04 & -72:50:58.4 & $17.834\pm0.009$ & $1.250\pm0.010$ & $190.24\pm0.30$ & $0.93$ & H \\
N419-1-b026 & 01:08:29.54 & -72:51:08.5 & $17.755\pm0.007$ & $0.905\pm0.009$ & $177.46\pm0.36$ & $0.00$ & H \\
N419-1-b027 & 01:08:33.47 & -72:51:17.0 & $18.714\pm0.009$ & $1.108\pm0.011$ & $112.31\pm0.63$ & $0.00$ & H \\
N419-1-b028 & 01:08:33.67 & -72:51:38.9 & $16.385\pm0.003$ & $1.766\pm0.004$ & $191.91\pm0.22$ & $0.72$ & H \\
N419-1-b029 & 01:08:38.81 & -72:51:45.7 & $16.818\pm0.004$ & $0.876\pm0.005$ & $146.89\pm0.27$ & $0.00$ & H \\
N419-1-b030 & 01:08:29.68 & -72:51:58.8 & $17.386\pm0.005$ & $1.340\pm0.006$ & $144.66\pm0.31$ & $0.00$ & H \\
N419-1-b031 & 01:08:35.45 & -72:52:05.2 & $18.612\pm0.008$ & $1.165\pm0.011$ & $132.97\pm0.63$ & $0.00$ & H \\
N419-1-b032 & 01:08:36.88 & -72:52:22.3 & $16.422\pm0.003$ & $1.680\pm0.004$ & $189.04\pm0.21$ & $0.94$ & H \\
N419-1-b033 & 01:08:28.67 & -72:59:24.5 & $18.561\pm0.036$ & $1.056\pm0.047$ & $172.83\pm0.56$ & $0.00$ & M \\
N419-1-b034 & 01:08:29.52 & -72:57:16.4 & $17.474\pm0.063$ & $1.323\pm0.115$ & $153.03\pm0.29$ & $0.00$ & M \\
N419-1-b035 & 01:08:27.14 & -72:54:05.2 & $17.010\pm0.005$ & $1.423\pm0.006$ & $188.55\pm0.22$ & $0.99$ & H \\
N419-1-b036 & 01:08:26.24 & -72:53:47.1 & $18.342\pm0.011$ & $1.124\pm0.015$ & $190.10\pm0.61$ & $0.99$ & H \\
N419-1-b037 & 01:08:30.79 & -72:53:30.9 & $17.477\pm0.005$ & $1.153\pm0.006$ & $188.48\pm0.29$ & $0.98$ & H \\
N419-1-b038 & 01:08:31.77 & -72:53:13.3 & $18.697\pm0.009$ & $0.946\pm0.012$ & $120.42\pm0.94$ & $0.00$ & H \\
N419-1-b039 & 01:08:28.43 & -72:53:12.6 & $18.621\pm0.009$ & $1.051\pm0.012$ & $187.58\pm0.79$ & $0.99$ & H \\
N419-1-b040 & 01:08:28.99 & -72:52:58.2 & $17.982\pm0.008$ & $1.163\pm0.009$ & $192.70\pm0.56$ & $0.97$ & H \\
N419-1-b041 & 01:08:33.26 & -73:00:25.3 & $17.997\pm0.106$ & $0.946\pm0.301$ & $189.95\pm0.46$ & $0.00$ & M \\
N419-1-b043 & 01:08:34.41 & -72:55:19.0 & $18.900\pm0.042$ & $1.034\pm0.068$ & $144.91\pm1.60$ & $0.00$ & M \\
N419-1-b046 & 01:08:34.51 & -72:52:59.8 & $15.918\pm0.002$ & $1.244\pm0.003$ & $182.92\pm0.17$ & $0.00$ & H \\
N419-1-b047 & 01:08:32.54 & -72:52:45.8 & $18.615\pm0.010$ & $1.082\pm0.012$ & $191.86\pm0.70$ & $0.97$ & H \\
N419-1-b048 & 01:08:36.71 & -72:52:40.4 & $18.329\pm0.007$ & $1.155\pm0.009$ & $171.83\pm0.40$ & $0.00$ & H \\
N419-1-b049 & 01:08:25.26 & -72:48:18.5 & $18.977\pm0.044$ & $0.885\pm0.092$ & $159.73\pm1.57$ & $0.00$ & M \\
N419-1-b050 & 01:08:22.58 & -72:51:11.8 & $18.949\pm0.026$ & $0.991\pm0.032$ & $139.76\pm1.13$ & $0.00$ & H \\
N419-1-b051 & 01:08:25.32 & -72:51:18.1 & $17.126\pm0.007$ & $1.438\pm0.008$ & $190.63\pm0.35$ & $0.93$ & H \\
N419-1-b052 & 01:08:22.12 & -72:51:37.8 & $17.296\pm0.005$ & $1.314\pm0.006$ & $197.80\pm0.28$ & $0.00$ & H \\
N419-1-b053 & 01:08:28.90 & -72:51:42.8 & $18.442\pm0.012$ & $0.855\pm0.016$ & $146.51\pm1.03$ & $0.00$ & H \\
N419-1-b055 & 01:08:24.75 & -72:52:25.3 & $17.717\pm0.008$ & $1.107\pm0.010$ & $192.58\pm0.45$ & $0.98$ & H \\
N419-1-b057 & 01:08:16.73 & -72:51:29.0 & $17.752\pm0.008$ & $1.364\pm0.009$ & $139.19\pm0.33$ & $0.00$ & H \\
N419-1-b058 & 01:08:17.65 & -72:51:52.8 & $16.563\pm0.003$ & $1.566\pm0.004$ & $188.98\pm0.20$ & $0.99$ & H \\
N419-1-b059 & 01:08:21.63 & -72:52:00.7 & $18.862\pm0.010$ & $0.958\pm0.013$ & $190.29\pm1.00$ & $0.99$ & H \\
N419-1-b061 & 01:08:20.37 & -72:52:22.1 & $16.785\pm0.004$ & $1.496\pm0.004$ & $188.40\pm0.25$ & $1.00$ & H \\
N419-1-b063 & 01:08:13.56 & -72:52:40.1 & $18.429\pm0.008$ & $1.051\pm0.010$ & $190.22\pm1.38$ & $1.00$ & H \\
N419-1-b064 & 01:08:17.60 & -72:52:48.4 & $18.092\pm0.008$ & $1.183\pm0.009$ & $189.78\pm2.07$ & $1.00$ & H \\
N419-1-b065 & 01:08:13.57 & -72:54:31.7 & $18.633\pm0.010$ & $1.140\pm0.013$ & $175.23\pm0.69$ & $0.00$ & H \\
N419-1-b066 & 01:08:10.42 & -72:54:16.5 & $18.245\pm0.009$ & $1.176\pm0.011$ & $142.15\pm0.57$ & $0.00$ & H \\
N419-1-b067 & 01:08:17.34 & -72:54:12.7 & $17.027\pm0.008$ & $1.445\pm0.011$ & $190.42\pm0.35$ & $0.99$ & H \\
N419-1-b069 & 01:08:14.49 & -72:53:31.4 & $17.865\pm0.006$ & $1.163\pm0.008$ & $187.93\pm0.63$ & $1.00$ & H \\
N419-1-b070 & 01:08:10.48 & -72:53:27.3 & $19.161\pm0.010$ & $0.916\pm0.014$ & $185.28\pm1.45$ & $1.00$ & H \\
N419-1-b071 & 01:08:14.04 & -72:53:16.4 & $16.573\pm0.003$ & $1.564\pm0.004$ & $187.81\pm0.37$ & $1.00$ & H \\
N419-1-b074 & 01:08:25.83 & -72:54:19.8 & $18.574\pm0.013$ & $1.063\pm0.017$ & $189.96\pm0.68$ & $0.96$ & H \\
N419-1-b075 & 01:08:21.22 & -72:54:03.6 & $17.017\pm0.004$ & $1.573\pm0.005$ & $161.88\pm0.30$ & $0.00$ & H \\
N419-1-b077 & 01:08:22.33 & -72:53:40.0 & $19.442\pm0.015$ & $0.903\pm0.019$ & $186.61\pm1.99$ & $1.00$ & H \\
N419-1-b078 & 01:08:24.57 & -72:53:28.2 & $17.418\pm0.005$ & $1.245\pm0.006$ & $189.61\pm0.34$ & $1.00$ & H \\
N419-1-b079 & 01:08:18.45 & -72:53:15.9 & $16.921\pm0.004$ & $1.387\pm0.005$ & $188.15\pm0.51$ & $1.00$ & H \\
N419-1-b080 & 01:08:19.35 & -72:53:00.9 & $16.422\pm0.003$ & $1.682\pm0.004$ & $189.50\pm0.62$ & $1.00$ & H \\
N419-1-b081 & 01:08:10.72 & -72:49:08.4 & $16.956\pm0.033$ & $1.321\pm0.276$ & $123.35\pm0.36$ & $0.00$ & M \\
N419-1-b082 & 01:08:13.42 & -72:51:11.0 & $18.842\pm0.011$ & $1.071\pm0.014$ & $189.78\pm0.93$ & $0.94$ & H \\
N419-1-b083 & 01:08:10.12 & -72:51:21.7 & $18.596\pm0.009$ & $1.093\pm0.012$ & $117.91\pm0.85$ & $0.00$ & H \\
N419-1-b084 & 01:08:12.53 & -72:51:30.2 & $17.660\pm0.006$ & $1.187\pm0.007$ & $191.81\pm0.29$ & $0.80$ & H \\
N419-1-b086 & 01:08:12.85 & -72:52:25.0 & $18.587\pm0.009$ & $0.880\pm0.012$ & $146.58\pm1.76$ & $0.00$ & H \\
N419-1-b087 & 01:08:09.31 & -72:52:37.5 & $16.944\pm0.005$ & $1.323\pm0.006$ & $192.62\pm0.34$ & $0.98$ & H \\
N419-1-b088 & 01:08:09.87 & -72:52:54.5 & $16.992\pm0.005$ & $1.413\pm0.006$ & $188.23\pm0.32$ & $1.00$ & H \\
N419-1-b089 & 01:08:06.74 & -72:51:17.8 & $18.399\pm0.011$ & $1.073\pm0.014$ & $189.03\pm0.50$ & $0.94$ & H \\
N419-1-b091 & 01:08:05.25 & -72:51:52.7 & $18.349\pm0.007$ & $1.069\pm0.009$ & $168.13\pm0.78$ & $0.00$ & H \\
N419-1-b092 & 01:08:08.77 & -72:51:55.3 & $19.021\pm0.012$ & $0.840\pm0.016$ & $184.36\pm2.47$ & $0.87$ & H \\
N419-1-b093 & 01:08:04.31 & -72:52:09.6 & $17.011\pm0.005$ & $1.323\pm0.006$ & $187.75\pm0.24$ & $0.97$ & H \\
N419-1-b094 & 01:08:05.31 & -72:52:30.0 & $16.772\pm0.004$ & $0.914\pm0.005$ & $157.41\pm0.29$ & $0.00$ & H \\
N419-1-b095 & 01:08:06.26 & -72:52:55.3 & $19.328\pm0.015$ & $0.901\pm0.019$ & $172.96\pm2.16$ & $0.00$ & H \\
N419-1-b096 & 01:08:07.57 & -72:53:10.7 & $17.097\pm0.006$ & $1.412\pm0.007$ & $188.48\pm0.24$ & $0.99$ & H \\
N419-1-b097 & 01:07:34.42 & -72:57:42.7 & $17.215\pm0.030$ & $0.956\pm0.055$ & $159.54\pm0.32$ & $0.00$ & M \\
N419-1-b098 & 01:07:33.01 & -72:57:06.7 & $16.802\pm0.050$ & $1.732\pm0.060$ & $175.10\pm0.27$ & $0.00$ & M \\
N419-1-b099 & 01:07:32.16 & -72:56:45.0 & $16.907\pm0.037$ & $1.542\pm0.129$ & $168.45\pm0.24$ & $0.00$ & M \\
N419-1-b100 & 01:07:46.32 & -72:56:03.5 & $17.036\pm0.033$ & $1.016\pm0.102$ & $191.41\pm0.25$ & $0.00$ & M \\
N419-1-b101 & 01:07:24.42 & -72:55:21.7 & $18.252\pm0.108$ & $1.212\pm0.122$ & $161.95\pm0.54$ & $0.00$ & M \\
N419-1-b102 & 01:06:54.30 & -72:55:17.1 & $17.468\pm0.029$ & $1.286\pm0.040$ & $146.65\pm0.37$ & $0.00$ & M \\
N419-1-b103 & 01:06:38.13 & -72:55:16.4 & $17.603\pm0.036$ & $1.365\pm0.271$ & $190.53\pm0.38$ & $0.00$ & M \\
N419-1-b104 & 01:07:31.81 & -72:54:00.3 & $17.507\pm0.187$ & $0.884\pm0.236$ & $151.85\pm0.37$ & $0.00$ & M \\
N419-1-b105 & 01:08:03.10 & -73:00:02.7 & $17.691\pm0.030$ & $1.408\pm0.077$ & $148.05\pm0.42$ & $0.00$ & M \\
N419-1-b106 & 01:07:51.35 & -72:58:01.4 & $18.800\pm0.102$ & $0.896\pm0.111$ & $182.85\pm1.67$ & $0.00$ & M \\
N419-1-b107 & 01:08:07.38 & -72:54:09.8 & $18.579\pm0.011$ & $1.129\pm0.013$ & $158.16\pm0.67$ & $0.00$ & H \\
N419-1-b109 & 01:08:06.35 & -72:53:32.4 & $16.666\pm0.004$ & $1.495\pm0.004$ & $190.11\pm0.24$ & $0.99$ & H \\
N419-1-b110 & 01:08:02.42 & -72:53:27.6 & $18.188\pm0.010$ & $1.140\pm0.013$ & $188.10\pm0.51$ & $0.98$ & H \\
N419-1-b111 & 01:08:04.02 & -72:53:10.5 & $17.301\pm0.007$ & $1.359\pm0.008$ & $190.28\pm0.34$ & $0.99$ & H \\
N419-1-b112 & 01:08:02.60 & -72:52:56.9 & $18.781\pm0.010$ & $1.011\pm0.013$ & $189.47\pm0.92$ & $0.99$ & H \\
N419-1-b114 & 01:07:51.42 & -72:50:55.6 & $16.972\pm0.029$ & $1.503\pm0.151$ & $161.58\pm0.25$ & $0.00$ & M \\
N419-1-b115 & 01:08:01.76 & -72:51:30.5 & $18.893\pm0.015$ & $0.797\pm0.018$ & $172.99\pm1.39$ & $0.00$ & H \\
N419-1-b117 & 01:07:29.46 & -72:52:04.5 & $18.969\pm0.036$ & $0.839\pm0.073$ & $131.08\pm1.48$ & $0.00$ & M \\
N419-1-b118 & 01:08:03.20 & -72:52:40.0 & $17.869\pm0.007$ & $1.142\pm0.009$ & $191.56\pm0.39$ & $0.98$ & H \\
N419-1-b119 & 01:07:53.96 & -72:54:06.2 & $18.464\pm0.031$ & $1.001\pm0.051$ & $159.17\pm0.50$ & $0.00$ & M \\
N419-1-b120 & 01:07:59.08 & -72:54:49.3 & $17.269\pm0.040$ & $1.394\pm0.056$ & $136.46\pm0.21$ & $0.00$ & M \\
N419-1-b121 & 01:07:30.01 & -72:49:42.7 & $17.971\pm0.031$ & $1.029\pm0.042$ & $142.66\pm0.65$ & $0.00$ & M \\
N419-1-b123 & 01:07:10.06 & -72:50:32.3 & $18.746\pm0.055$ & $0.889\pm0.091$ & $191.94\pm1.46$ & $0.00$ & M \\
N419-1-b124 & 01:07:22.03 & -72:50:49.3 & $18.413\pm0.036$ & $1.115\pm0.047$ & $166.43\pm0.60$ & $0.00$ & M \\
N419-1-b126 & 01:06:48.72 & -72:53:33.3 & $16.916\pm0.028$ & $1.015\pm0.040$ & $149.91\pm0.29$ & $0.00$ & M \\
N419-1-b127 & 01:06:36.00 & -72:54:14.6 & $17.088\pm0.032$ & $1.284\pm0.049$ & $141.47\pm1.12$ & $0.00$ & M \\
N419-1-b128 & 01:06:59.45 & -72:54:39.6 & $16.997\pm0.030$ & $1.372\pm0.064$ & $142.84\pm0.28$ & $0.00$ & M \\
N419-1-r049 & 01:08:14.47 & -72:53:56.6 & $16.214\pm0.004$ & $1.934\pm0.004$ & $186.85\pm0.36$ & $0.97$ & H \\
N419-1-r079 & 01:08:20.73 & -72:52:47.2 & $16.342\pm0.003$ & $1.762\pm0.004$ & $193.99\pm0.29$ & $1.00$ & H \\
N419-1-r099 & 01:08:26.87 & -72:52:46.3 & $16.523\pm0.004$ & $1.661\pm0.004$ & $191.02\pm0.24$ & $0.99$ & H \\
N419-1-r127 & 01:08:23.70 & -72:53:09.1 & $16.312\pm0.003$ & $1.741\pm0.004$ & $187.89\pm0.40$ & $1.00$ & H \\
\hline
\end{tabular}
\begin{tablenotes}
 \item $^{\rm a}$ {Photometric source that the target were selected from: H stands for \textit{HST} and M stands for MCPS.}
\end{tablenotes}
\end{threeparttable}
\end{table*}


==> tab/t5_full.tex <==
\begin{table*}
\caption{Combined Sample of NGC 1846.}
\label{tab:sample_n1846}
\begin{threeparttable}
\begin{tabular}{ccccccccc}
\hline
{ID} & {$\alpha_{2000}$} & {$\delta_{2000}$} & {$V$} & {$V-I$} & {$v_{\rm los}$} & {$P_{M_i}$} & {Sel. $^{\rm a}$} & {Spec. $^{\rm b}$} \\
{} & {(h:m:s)} & {($^{\circ}$:$\arcmin$:$\arcsec$)} & {(mag)} & {(mag)} & {(km\,s$^{-1}$)} &  {} & {} & {} \\
\hline
N1846-1-b001 & 05:07:51.21 & -67:33:03.8 & $17.251\pm0.307$ & $1.396\pm0.310$ & $287.97\pm0.19$ & $0.00$ & M & M2FS \\
N1846-1-b002 & 05:07:57.56 & -67:32:58.0 & $17.314\pm0.049$ & $1.266\pm0.069$ & $264.51\pm0.19$ & $0.00$ & M & M2FS \\
N1846-1-b003 & 05:07:49.91 & -67:32:21.2 & $17.559\pm0.041$ & $1.255\pm0.058$ & $246.95\pm0.18$ & $0.00$ & M & M2FS \\
N1846-1-b005 & 05:07:54.32 & -67:30:17.6 & $17.715\pm0.030$ & $1.192\pm0.050$ & $221.35\pm0.23$ & $0.00$ & M & M2FS \\
N1846-1-b006 & 05:07:47.87 & -67:29:52.6 & $17.329\pm0.028$ & $1.345\pm0.049$ & $271.34\pm0.19$ & $0.00$ & M & M2FS \\
N1846-1-b007 & 05:07:56.92 & -67:29:28.9 & $17.387\pm0.146$ & $1.256\pm0.151$ & $286.79\pm0.20$ & $0.00$ & M & M2FS \\
N1846-1-b009 & 05:08:21.28 & -67:31:11.1 & $17.125\pm0.026$ & $1.301\pm0.049$ & $287.38\pm0.17$ & $0.00$ & M & M2FS \\
N1846-1-b010 & 05:08:29.24 & -67:31:03.5 & $17.475\pm0.050$ & $1.278\pm0.071$ & $231.89\pm0.18$ & $0.00$ & M & M2FS \\
N1846-1-b011 & 05:08:24.35 & -67:30:58.2 & $17.212\pm0.054$ & $1.304\pm0.067$ & $275.75\pm0.18$ & $0.00$ & M & M2FS \\
N1846-1-b012 & 05:08:30.22 & -67:30:34.4 & $17.595\pm0.060$ & $1.194\pm0.076$ & $274.73\pm0.19$ & $0.00$ & M & M2FS \\
N1846-1-b013 & 05:08:10.21 & -67:29:55.3 & $17.508\pm0.038$ & $1.348\pm0.055$ & $216.72\pm0.20$ & $0.00$ & M & M2FS \\
N1846-1-b015 & 05:08:34.55 & -67:29:23.9 & $17.601\pm0.031$ & $1.284\pm0.051$ & $271.05\pm0.20$ & $0.00$ & M & M2FS \\
N1846-1-b016 & 05:08:44.83 & -67:29:05.7 & $17.668\pm0.043$ & $1.178\pm0.069$ & $273.20\pm0.21$ & $0.00$ & M & M2FS \\
N1846-1-b017 & 05:08:18.68 & -67:24:42.1 & $17.657\pm0.031$ & $1.293\pm0.051$ & $272.52\pm0.24$ & $0.00$ & M & M2FS \\
N1846-1-b019 & 05:08:39.28 & -67:25:53.4 & $17.271\pm0.023$ & $1.354\pm0.046$ & $318.50\pm0.14$ & $0.00$ & M & M2FS \\
N1846-1-b020 & 05:08:16.63 & -67:27:13.4 & $17.627\pm0.039$ & $1.228\pm0.078$ & $274.40\pm0.15$ & $0.00$ & M & M2FS \\
N1846-1-b021 & 05:08:41.57 & -67:27:26.0 & $17.651\pm0.053$ & $1.184\pm0.071$ & $308.68\pm0.30$ & $0.00$ & M & M2FS \\
N1846-1-b022 & 05:08:39.60 & -67:27:39.3 & $17.530\pm0.031$ & $1.297\pm0.054$ & $276.49\pm0.19$ & $0.00$ & M & M2FS \\
N1846-1-b023 & 05:08:17.46 & -67:27:44.8 & $17.106\pm0.027$ & $1.295\pm0.048$ & $277.78\pm0.15$ & $0.00$ & M & M2FS \\
N1846-1-b025 & 05:08:08.02 & -67:22:52.5 & $17.726\pm0.242$ & $1.295\pm0.246$ & $228.47\pm0.21$ & $0.00$ & M & M2FS \\
N1846-1-b027 & 05:08:10.54 & -67:24:20.9 & $17.619\pm0.031$ & $1.180\pm0.051$ & $249.71\pm0.20$ & $0.00$ & M & M2FS \\
N1846-1-b030 & 05:07:50.87 & -67:26:13.7 & $17.515\pm0.031$ & $1.283\pm0.051$ & $268.99\pm0.19$ & $0.00$ & M & M2FS \\
N1846-1-b031 & 05:08:08.63 & -67:26:24.4 & $17.135\pm0.031$ & $1.323\pm0.051$ & $281.85\pm0.14$ & $0.00$ & M & M2FS \\
N1846-1-b032 & 05:08:06.22 & -67:27:24.2 & $17.569\pm0.035$ & $1.327\pm0.055$ & $256.58\pm0.19$ & $0.00$ & M & M2FS \\
N1846-1-b033 & 05:07:36.65 & -67:30:16.5 & $18.191\pm0.008$ & $1.141\pm0.012$ & $284.64\pm0.32$ & $0.00$ & H & M2FS \\
N1846-1-b034 & 05:07:39.86 & -67:29:04.6 & $17.828\pm0.031$ & $1.140\pm0.074$ & $239.85\pm0.27$ & $0.96$ & M & M2FS \\
N1846-1-b035 & 05:07:40.01 & -67:28:31.2 & $17.944\pm0.006$ & $1.164\pm0.010$ & $237.57\pm0.23$ & $0.99$ & H & M2FS \\
N1846-1-b036 & 05:07:38.41 & -67:28:11.9 & $17.097\pm0.004$ & $1.431\pm0.006$ & $237.02\pm0.18$ & $1.00$ & H & COMB \\
N1846-1-b037 & 05:07:36.12 & -67:28:07.8 & $17.872\pm0.006$ & $1.223\pm0.009$ & $238.59\pm0.21$ & $1.00$ & H & M2FS \\
N1846-1-b038 & 05:07:38.15 & -67:27:58.7 & $17.345\pm0.005$ & $1.346\pm0.007$ & $237.39\pm0.22$ & $1.00$ & H & M2FS \\
N1846-1-b039 & 05:07:39.58 & -67:27:38.2 & $17.223\pm0.006$ & $1.368\pm0.008$ & $238.69\pm0.21$ & $1.00$ & H & M2FS \\
N1846-1-b043 & 05:07:42.35 & -67:28:46.1 & $18.248\pm0.008$ & $1.069\pm0.015$ & $245.91\pm0.54$ & $0.00$ & H & M2FS \\
N1846-1-b044 & 05:07:45.51 & -67:28:34.2 & $18.077\pm0.008$ & $1.130\pm0.012$ & $264.15\pm0.23$ & $0.00$ & H & M2FS \\
N1846-1-b045 & 05:07:47.37 & -67:28:19.8 & $17.580\pm0.007$ & $1.191\pm0.011$ & $236.37\pm0.29$ & $0.61$ & H & M2FS \\
N1846-1-b046 & 05:07:44.74 & -67:28:18.5 & $17.078\pm0.005$ & $1.378\pm0.007$ & $237.50\pm0.17$ & $0.99$ & H & M2FS \\
N1846-1-b047 & 05:07:43.71 & -67:27:58.4 & $18.138\pm0.008$ & $1.119\pm0.012$ & $238.06\pm0.29$ & $1.00$ & H & M2FS \\
N1846-1-b048 & 05:07:41.77 & -67:27:51.3 & $18.301\pm0.008$ & $1.119\pm0.012$ & $240.36\pm0.32$ & $1.00$ & H & M2FS \\
N1846-1-b049 & 05:07:42.99 & -67:21:35.8 & $17.481\pm0.031$ & $1.321\pm0.040$ & $271.34\pm0.25$ & $0.00$ & M & M2FS \\
N1846-1-b050 & 05:07:45.88 & -67:23:42.5 & $17.471\pm0.034$ & $1.260\pm0.110$ & $282.03\pm0.21$ & $0.00$ & M & M2FS \\
N1846-1-b052 & 05:07:47.67 & -67:26:05.6 & $17.546\pm0.033$ & $1.317\pm0.053$ & $236.68\pm0.21$ & $0.27$ & M & M2FS \\
N1846-1-b053 & 05:07:41.62 & -67:26:27.4 & $18.302\pm0.050$ & $1.107\pm0.068$ & $280.18\pm0.31$ & $0.00$ & M & M2FS \\
N1846-1-b054 & 05:07:37.75 & -67:26:51.9 & $17.956\pm0.006$ & $1.135\pm0.012$ & $237.89\pm0.27$ & $1.00$ & H & M2FS \\
N1846-1-b055 & 05:07:39.46 & -67:26:59.9 & $18.292\pm0.006$ & $1.086\pm0.011$ & $238.90\pm0.28$ & $1.00$ & H & M2FS \\
N1846-1-b056 & 05:07:40.73 & -67:27:22.2 & $17.760\pm0.005$ & $1.148\pm0.009$ & $239.49\pm0.22$ & $1.00$ & H & M2FS \\
N1846-1-b057 & 05:07:33.97 & -67:22:12.1 & $17.608\pm0.043$ & $1.266\pm0.050$ & $240.19\pm0.25$ & $0.00$ & M & M2FS \\
N1846-1-b058 & 05:07:32.31 & -67:26:35.3 & $17.770\pm0.007$ & $1.182\pm0.010$ & $239.90\pm0.22$ & $1.00$ & H & M2FS \\
N1846-1-b059 & 05:07:32.45 & -67:26:49.6 & $17.398\pm0.008$ & $1.252\pm0.010$ & $240.29\pm0.26$ & $1.00$ & H & M2FS \\
N1846-1-b061 & 05:07:34.81 & -67:26:53.6 & $17.504\pm0.010$ & $1.249\pm0.012$ & $241.38\pm0.21$ & $1.00$ & H & M2FS \\
N1846-1-b062 & 05:07:34.27 & -67:27:13.7 & $17.541\pm0.005$ & $1.305\pm0.008$ & $243.18\pm0.23$ & $0.99$ & H & M2FS \\
N1846-1-b063 & 05:07:36.86 & -67:27:19.2 & $18.201\pm0.006$ & $1.127\pm0.011$ & $242.08\pm0.24$ & $1.00$ & H & M2FS \\
N1846-1-b064 & 05:07:34.23 & -67:27:27.0 & $17.624\pm0.007$ & $1.197\pm0.009$ & $239.50\pm0.31$ & $1.00$ & H & M2FS \\
N1846-1-b065 & 05:07:22.62 & -67:33:31.4 & $17.170\pm0.048$ & $1.340\pm0.070$ & $314.15\pm0.19$ & $0.00$ & M & M2FS \\
N1846-1-b066 & 05:07:28.51 & -67:32:40.7 & $17.527\pm0.031$ & $1.225\pm0.061$ & $268.08\pm0.29$ & $0.00$ & M & M2FS \\
N1846-1-b067 & 05:07:29.05 & -67:31:58.0 & $17.503\pm0.033$ & $1.354\pm0.053$ & $290.41\pm0.85$ & $0.00$ & M & M2FS \\
N1846-1-b068 & 05:07:30.38 & -67:29:36.0 & $17.617\pm0.006$ & $1.237\pm0.008$ & $239.36\pm0.16$ & $0.97$ & H & COMB \\
N1846-1-b069 & 05:07:27.44 & -67:29:27.9 & $17.881\pm0.006$ & $1.124\pm0.010$ & $238.88\pm0.21$ & $0.97$ & H & COMB \\
N1846-1-b070 & 05:07:29.52 & -67:28:48.8 & $18.291\pm0.008$ & $1.158\pm0.013$ & $240.42\pm0.32$ & $1.00$ & H & M2FS \\
N1846-1-b071 & 05:07:28.71 & -67:28:24.7 & $17.516\pm0.007$ & $1.199\pm0.010$ & $238.60\pm0.19$ & $1.00$ & H & COMB \\
N1846-1-b072 & 05:07:26.13 & -67:28:08.3 & $17.878\pm0.006$ & $1.203\pm0.009$ & $240.45\pm0.25$ & $1.00$ & H & M2FS \\
N1846-1-b073 & 05:07:32.70 & -67:30:37.3 & $18.404\pm0.021$ & $1.123\pm0.025$ & $272.60\pm0.25$ & $0.00$ & H & M2FS \\
N1846-1-b074 & 05:07:32.36 & -67:29:22.1 & $18.387\pm0.010$ & $1.011\pm0.016$ & $286.00\pm0.33$ & $0.00$ & H & M2FS \\
N1846-1-b075 & 05:07:31.11 & -67:29:06.2 & $18.162\pm0.006$ & $1.112\pm0.011$ & $237.78\pm0.27$ & $0.92$ & H & M2FS \\
N1846-1-b076 & 05:07:34.98 & -67:28:54.9 & $17.514\pm0.006$ & $1.338\pm0.009$ & $281.13\pm0.21$ & $0.00$ & H & M2FS \\
N1846-1-b077 & 05:07:34.52 & -67:28:24.5 & $17.849\pm0.008$ & $1.236\pm0.011$ & $239.55\pm0.27$ & $1.00$ & H & COMB \\
N1846-1-b078 & 05:07:34.01 & -67:28:10.7 & $18.325\pm0.006$ & $1.051\pm0.012$ & $241.18\pm0.36$ & $1.00$ & H & M2FS \\
N1846-1-b079 & 05:07:30.42 & -67:28:04.5 & $17.090\pm0.005$ & $1.367\pm0.007$ & $239.58\pm0.17$ & $1.00$ & H & COMB \\
N1846-1-b080 & 05:07:34.59 & -67:27:55.7 & $17.289\pm0.005$ & $1.329\pm0.007$ & $259.98\pm0.22$ & $0.00$ & H & M2FS \\
N1846-1-b081 & 05:07:27.72 & -67:20:59.1 & $17.354\pm0.051$ & $1.283\pm0.058$ & $272.38\pm0.21$ & $0.00$ & M & M2FS \\
N1846-1-b082 & 05:07:29.23 & -67:25:09.4 & $17.542\pm0.033$ & $1.176\pm0.055$ & $273.57\pm0.25$ & $0.00$ & M & M2FS \\
N1846-1-b083 & 05:07:29.61 & -67:26:27.7 & $17.914\pm0.008$ & $1.231\pm0.011$ & $242.93\pm0.26$ & $0.33$ & H & COMB \\
N1846-1-b084 & 05:07:30.03 & -67:26:43.0 & $17.175\pm0.005$ & $1.341\pm0.007$ & $239.37\pm0.18$ & $1.00$ & H & COMB \\
N1846-1-b085 & 05:07:29.78 & -67:26:57.3 & $18.303\pm0.011$ & $1.088\pm0.015$ & $238.90\pm0.32$ & $1.00$ & H & M2FS \\
N1846-1-b087 & 05:07:32.10 & -67:27:20.1 & $17.303\pm0.006$ & $1.357\pm0.008$ & $239.89\pm0.22$ & $1.00$ & H & M2FS \\
N1846-1-b088 & 05:07:27.74 & -67:27:30.5 & $17.389\pm0.006$ & $1.276\pm0.008$ & $238.90\pm0.21$ & $1.00$ & H & M2FS \\
N1846-1-b089 & 05:07:27.31 & -67:23:08.7 & $17.222\pm0.084$ & $1.409\pm0.142$ & $209.72\pm0.20$ & $0.00$ & M & M2FS \\
N1846-1-b090 & 05:07:23.74 & -67:26:32.8 & $17.862\pm0.006$ & $1.176\pm0.010$ & $271.38\pm0.24$ & $0.00$ & H & M2FS \\
N1846-1-b092 & 05:07:23.62 & -67:26:50.9 & $17.337\pm0.007$ & $1.363\pm0.009$ & $263.45\pm0.20$ & $0.00$ & H & COMB \\
N1846-1-b093 & 05:07:26.29 & -67:26:57.1 & $18.010\pm0.006$ & $1.167\pm0.010$ & $292.12\pm0.26$ & $0.00$ & H & COMB \\
N1846-1-b094 & 05:07:21.17 & -67:27:01.6 & $17.157\pm0.004$ & $1.368\pm0.006$ & $249.96\pm0.17$ & $0.00$ & H & COMB \\
N1846-1-b095 & 05:07:24.90 & -67:27:14.0 & $18.363\pm0.008$ & $1.023\pm0.013$ & $235.76\pm0.29$ & $0.99$ & H & M2FS \\
N1846-1-b096 & 05:07:21.66 & -67:27:25.7 & $17.603\pm0.005$ & $1.270\pm0.008$ & $240.15\pm0.21$ & $1.00$ & H & COMB \\
N1846-1-b097 & 05:06:41.49 & -67:30:29.3 & $17.523\pm0.048$ & $1.259\pm0.069$ & $264.60\pm0.37$ & $0.00$ & M & M2FS \\
N1846-1-b098 & 05:07:04.08 & -67:30:27.1 & $17.316\pm0.121$ & $1.251\pm0.127$ & $315.36\pm0.22$ & $0.00$ & M & M2FS \\
N1846-1-b099 & 05:06:26.99 & -67:29:46.2 & $17.652\pm0.055$ & $1.242\pm0.071$ & $250.96\pm0.36$ & $0.00$ & M & M2FS \\
N1846-1-b100 & 05:07:06.54 & -67:29:29.4 & $17.172\pm0.108$ & $1.302\pm0.116$ & $316.04\pm0.19$ & $0.00$ & M & M2FS \\
N1846-1-b101 & 05:07:14.70 & -67:29:16.2 & $17.535\pm0.011$ & $1.335\pm0.013$ & $280.36\pm0.19$ & $0.00$ & H & COMB \\
N1846-1-b102 & 05:07:10.60 & -67:28:31.4 & $18.059\pm0.008$ & $1.166\pm0.012$ & $280.89\pm0.25$ & $0.00$ & H & COMB \\
N1846-1-b103 & 05:07:12.27 & -67:28:03.4 & $18.374\pm0.007$ & $1.157\pm0.011$ & $277.60\pm0.27$ & $0.00$ & H & M2FS \\
N1846-1-b104 & 05:07:14.42 & -67:27:48.4 & $18.118\pm0.010$ & $1.184\pm0.013$ & $290.83\pm0.20$ & $0.00$ & H & COMB \\
N1846-1-b105 & 05:07:21.53 & -67:34:28.6 & $17.266\pm0.036$ & $1.396\pm0.060$ & $275.00\pm0.27$ & $0.00$ & M & M2FS \\
N1846-1-b106 & 05:07:17.39 & -67:33:22.2 & $17.688\pm0.037$ & $1.215\pm0.055$ & $274.33\pm0.24$ & $0.00$ & M & M2FS \\
N1846-1-b110 & 05:07:19.98 & -67:29:37.3 & $17.423\pm0.004$ & $1.340\pm0.007$ & $310.81\pm0.15$ & $0.00$ & H & COMB \\
N1846-1-b111 & 05:07:22.21 & -67:28:01.1 & $18.459\pm0.009$ & $1.049\pm0.015$ & $240.13\pm0.37$ & $1.00$ & H & M2FS \\
N1846-1-b112 & 05:07:21.79 & -67:27:48.3 & $17.254\pm0.004$ & $1.278\pm0.006$ & $240.07\pm0.23$ & $1.00$ & H & M2FS \\
N1846-1-b114 & 05:07:14.72 & -67:22:39.4 & $17.653\pm0.033$ & $1.218\pm0.054$ & $288.47\pm0.22$ & $0.00$ & M & M2FS \\
N1846-1-b118 & 05:07:20.90 & -67:25:42.3 & $17.657\pm0.085$ & $1.197\pm0.095$ & $239.63\pm0.26$ & $0.96$ & M & M2FS \\
N1846-1-b119 & 05:07:19.94 & -67:26:33.8 & $17.607\pm0.049$ & $1.189\pm0.075$ & $234.77\pm0.23$ & $0.00$ & M & M2FS \\
N1846-1-b120 & 05:07:17.91 & -67:27:12.2 & $17.388\pm0.137$ & $1.359\pm0.143$ & $239.45\pm0.21$ & $0.96$ & M & M2FS \\
N1846-1-b121 & 05:06:59.17 & -67:23:06.7 & $17.024\pm0.023$ & $1.295\pm0.080$ & $251.92\pm0.19$ & $0.00$ & M & M2FS \\
N1846-1-b122 & 05:06:32.56 & -67:24:21.3 & $17.646\pm0.044$ & $1.188\pm0.063$ & $245.75\pm0.30$ & $0.00$ & M & M2FS \\
N1846-1-b123 & 05:06:58.93 & -67:24:28.2 & $17.437\pm0.085$ & $1.210\pm0.105$ & $250.13\pm0.22$ & $0.00$ & M & M2FS \\
N1846-1-b126 & 05:06:31.87 & -67:26:14.9 & $17.533\pm0.031$ & $1.262\pm0.052$ & $214.26\pm0.34$ & $0.00$ & M & M2FS \\
N1846-1-b127 & 05:06:48.68 & -67:27:11.0 & $17.611\pm0.099$ & $1.301\pm0.109$ & $250.71\pm1.47$ & $0.00$ & M & M2FS \\
N1846-1-b128 & 05:06:39.18 & -67:27:36.1 & $17.460\pm0.031$ & $1.211\pm0.053$ & $289.27\pm0.51$ & $0.00$ & M & M2FS \\
N1846-1-r049 & 05:07:32.21 & -67:27:51.6 & $17.154\pm0.004$ & $1.401\pm0.006$ & $241.93\pm0.26$ & $1.00$ & H & M2FS \\
N1846-1-r079 & 05:07:30.12 & -67:27:27.7 & $17.115\pm0.004$ & $1.306\pm0.006$ & $238.29\pm0.17$ & $1.00$ & H & COMB \\
N1846-1-r099 & 05:07:31.18 & -67:27:39.9 & $17.054\pm0.004$ & $1.422\pm0.006$ & $239.11\pm0.19$ & $1.00$ & H & M2FS \\
N1846-1-r127 & 05:07:34.13 & -67:27:43.3 & $17.057\pm0.004$ & $1.336\pm0.006$ & $239.22\pm0.20$ & $1.00$ & H & M2FS \\
ACS-001-R & 05:07:36.84 & -67:27:45.9 & $16.56$ & $1.70$ & $236.11\pm0.53$ & $1.00$ & H & M13 \\
ACS-013-R & 05:07:33.59 & -67:26:41.2 & $16.99$ & $1.43$ & $238.10\pm0.46$ & $1.00$ & H & M13 \\
ACS-019-R & 05:07:14.49 & -67:28:16.4 & ... & ... & $278.73\pm0.47$ & $0.00$ & H & M13 \\
ACS-025-R & 05:07:36.19 & -67:27:58.8 & $17.28$ & $1.35$ & $238.28\pm0.49$ & $1.00$ & H & M13 \\
ACS-030-R & 05:07:39.01 & -67:28:23.2 & $17.43$ & $1.31$ & $240.65\pm0.60$ & $1.00$ & H & M13 \\
ACS-046-R & 05:07:32.64 & -67:27:45.5 & $17.92$ & $1.24$ & $237.54\pm0.62$ & $1.00$ & H & M13 \\
ACS-051-R & 05:07:36.60 & -67:27:33.5 & $17.96$ & $1.25$ & $235.60\pm0.77$ & $1.00$ & H & M13 \\
ACS-059-R & 05:07:28.63 & -67:28:44.8 & $18.04$ & $1.19$ & $237.75\pm0.77$ & $1.00$ & H & M13 \\
ACS-066-R & 05:07:49.57 & -67:29:01.4 & $18.18$ & $1.18$ & $239.43\pm0.78$ & $0.96$ & H & M13 \\
ACS-080-A & 05:07:30.30 & -67:27:11.2 & $17.09$ & $1.36$ & $243.87\pm0.47$ & $0.92$ & H & M13 \\
ACS-090-A & 05:07:30.17 & -67:27:46.1 & $17.53$ & $1.24$ & $238.02\pm0.62$ & $1.00$ & H & M13 \\
ACS-112-A & 05:07:43.29 & -67:26:49.9 & $18.02$ & $1.12$ & $239.80\pm0.67$ & $0.96$ & H & M13 \\
MCPS-007 & 05:05:34.36 & -67:26:34.2 & $16.810\pm0.063$ & $1.622\pm0.079$ & $253.77\pm0.85$ & $0.00$ & M & M13 \\
MCPS-010 & 05:05:40.15 & -67:24:55.8 & $16.820\pm0.048$ & $1.792\pm0.063$ & $265.39\pm0.59$ & $0.00$ & M & M13 \\
MCPS-016 & 05:05:48.25 & -67:26:42.0 & $16.622\pm0.191$ & $1.636\pm0.195$ & $277.40\pm0.55$ & $0.00$ & M & M13 \\
MCPS-017 & 05:05:48.26 & -67:34:31.0 & $16.868\pm0.027$ & $1.553\pm0.047$ & $305.87\pm0.59$ & $0.00$ & M & M13 \\
MCPS-018 & 05:05:49.11 & -67:24:18.3 & $16.586\pm0.065$ & $2.020\pm0.076$ & $271.71\pm1.03$ & $0.00$ & M & M13 \\
MCPS-021 & 05:05:55.85 & -67:36:24.1 & $17.015\pm0.025$ & $1.955\pm0.052$ & $258.14\pm0.95$ & $0.00$ & M & M13 \\
MCPS-022 & 05:05:56.49 & -67:34:03.0 & $16.537\pm0.027$ & $1.533\pm0.047$ & $279.70\pm0.48$ & $0.00$ & M & M13 \\
MCPS-023 & 05:05:56.77 & -67:31:03.9 & $16.619\pm0.033$ & $1.724\pm0.053$ & $250.79\pm0.52$ & $0.00$ & M & M13 \\
MCPS-026 & 05:06:01.14 & -67:25:34.9 & $16.452\pm0.045$ & $1.810\pm0.060$ & $298.23\pm0.57$ & $0.00$ & M & M13 \\
MCPS-027 & 05:06:03.18 & -67:28:46.3 & $16.855\pm0.029$ & $1.576\pm0.049$ & $279.19\pm0.55$ & $0.00$ & M & M13 \\
MCPS-029 & 05:06:04.64 & -67:34:09.3 & $16.687\pm0.038$ & $1.684\pm0.064$ & $234.91\pm0.63$ & $0.00$ & M & M13 \\
MCPS-031 & 05:06:06.29 & -67:33:19.8 & $16.406\pm0.071$ & $1.694\pm0.087$ & $285.55\pm0.65$ & $0.00$ & M & M13 \\
MCPS-033 & 05:06:07.79 & -67:30:26.5 & $16.857\pm0.043$ & $1.544\pm0.059$ & $270.06\pm0.52$ & $0.00$ & M & M13 \\
MCPS-035 & 05:06:12.98 & -67:28:56.5 & $16.732\pm0.034$ & $1.730\pm0.055$ & $259.76\pm0.45$ & $0.00$ & M & M13 \\
MCPS-038 & 05:06:16.30 & -67:30:11.6 & $16.652\pm0.031$ & $1.927\pm0.049$ & $235.10\pm0.59$ & $0.00$ & M & M13 \\
MCPS-040 & 05:06:17.30 & -67:31:45.0 & $16.762\pm0.050$ & $1.714\pm0.066$ & $278.87\pm0.59$ & $0.00$ & M & M13 \\
MCPS-042 & 05:06:21.14 & -67:19:38.1 & $16.737\pm0.053$ & $1.748\pm0.058$ & $298.96\pm0.55$ & $0.00$ & M & M13 \\
MCPS-043 & 05:06:22.02 & -67:28:51.5 & $16.834\pm0.100$ & $1.688\pm0.107$ & $264.66\pm0.45$ & $0.00$ & M & M13 \\
MCPS-044 & 05:06:26.23 & -67:21:24.0 & $16.601\pm0.043$ & $1.768\pm0.051$ & $278.44\pm0.63$ & $0.00$ & M & M13 \\
MCPS-045 & 05:06:26.70 & -67:29:36.1 & $16.463\pm0.042$ & $1.772\pm0.057$ & $311.54\pm0.45$ & $0.00$ & M & M13 \\
MCPS-047 & 05:06:29.38 & -67:32:50.0 & $16.731\pm0.032$ & $1.628\pm0.050$ & $257.38\pm0.55$ & $0.00$ & M & M13 \\
MCPS-048 & 05:06:29.78 & -67:23:06.5 & $16.635\pm0.028$ & $1.719\pm0.050$ & $273.60\pm0.47$ & $0.00$ & M & M13 \\
MCPS-049 & 05:06:30.15 & -67:29:54.4 & $16.547\pm0.045$ & $1.661\pm0.065$ & $252.78\pm0.54$ & $0.00$ & M & M13 \\
MCPS-050 & 05:06:32.18 & -67:21:02.1 & $16.887\pm0.032$ & $1.731\pm0.051$ & $261.66\pm0.49$ & $0.00$ & M & M13 \\
MCPS-051 & 05:06:34.01 & -67:37:13.8 & $16.689\pm0.031$ & $1.679\pm0.051$ & $279.60\pm0.62$ & $0.00$ & M & M13 \\
MCPS-052 & 05:06:34.74 & -67:21:09.6 & $16.317\pm0.023$ & $1.784\pm0.033$ & $235.45\pm0.60$ & $0.00$ & M & M13 \\
MCPS-058 & 05:06:40.72 & -67:37:16.7 & $15.643\pm0.038$ & $1.445\pm0.055$ & $298.75\pm0.48$ & $0.00$ & M & M13 \\
MCPS-059 & 05:06:40.76 & -67:16:24.3 & $17.147\pm0.027$ & $1.765\pm0.036$ & $324.81\pm0.65$ & $0.00$ & M & M13 \\
MCPS-060 & 05:06:42.46 & -67:32:28.6 & $16.804\pm0.046$ & $1.979\pm0.060$ & $248.33\pm1.12$ & $0.00$ & M & M13 \\
MCPS-064 & 05:06:45.79 & -67:18:23.9 & $16.706\pm0.091$ & $1.778\pm0.104$ & $271.83\pm0.54$ & $0.00$ & M & M13 \\
MCPS-066 & 05:06:50.42 & -67:17:35.3 & $16.561\pm0.021$ & $1.535\pm0.032$ & $273.43\pm0.72$ & $0.00$ & M & M13 \\
MCPS-067 & 05:06:51.17 & -67:36:00.7 & $16.463\pm0.090$ & $1.691\pm0.104$ & $294.50\pm0.51$ & $0.00$ & M & M13 \\
MCPS-070 & 05:06:53.80 & -67:38:02.3 & $16.586\pm0.024$ & $1.802\pm0.047$ & $226.58\pm0.57$ & $0.00$ & M & M13 \\
MCPS-071 & 05:06:57.88 & -67:17:13.5 & $16.403\pm0.026$ & $1.895\pm0.036$ & $260.83\pm0.54$ & $0.00$ & M & M13 \\
MCPS-074 & 05:07:01.90 & -67:19:20.7 & $16.718\pm0.026$ & $1.685\pm0.036$ & $287.22\pm0.58$ & $0.00$ & M & M13 \\
MCPS-075 & 05:07:03.10 & -67:19:53.2 & $16.650\pm0.027$ & $1.505\pm0.037$ & $237.56\pm0.52$ & $0.00$ & M & M13 \\
MCPS-076 & 05:07:07.28 & -67:35:51.3 & $16.745\pm0.037$ & $1.583\pm0.054$ & $263.83\pm0.51$ & $0.00$ & M & M13 \\
MCPS-078 & 05:07:10.43 & -67:37:17.1 & $16.799\pm0.029$ & $1.923\pm0.050$ & $310.96\pm0.70$ & $0.00$ & M & M13 \\
MCPS-079 & 05:07:10.53 & -67:39:57.4 & $16.680\pm0.029$ & $1.803\pm0.049$ & $290.05\pm0.67$ & $0.00$ & M & M13 \\
MCPS-082 & 05:07:14.56 & -67:15:30.5 & $16.693\pm0.031$ & $1.532\pm0.056$ & $271.07\pm0.62$ & $0.00$ & M & M13 \\
MCPS-084 & 05:07:16.07 & -67:37:32.4 & $16.806\pm0.025$ & $1.832\pm0.049$ & $243.43\pm0.65$ & $0.00$ & M & M13 \\
MCPS-089 & 05:07:21.71 & -67:36:39.0 & $16.477\pm0.116$ & $1.639\pm0.123$ & $249.40\pm0.45$ & $0.00$ & M & M13 \\
MCPS-091 & 05:07:22.26 & -67:39:49.8 & $16.726\pm0.026$ & $1.877\pm0.047$ & $239.79\pm0.55$ & $0.00$ & M & M13 \\
MCPS-094 & 05:07:24.04 & -67:17:29.1 & $16.856\pm0.026$ & $1.610\pm0.037$ & $247.63\pm0.54$ & $0.00$ & M & M13 \\
MCPS-096 & 05:07:32.79 & -67:17:35.6 & $16.536\pm0.046$ & $1.857\pm0.053$ & $311.32\pm0.55$ & $0.00$ & M & M13 \\
MCPS-103 & 05:07:39.28 & -67:35:41.8 & $17.082\pm0.027$ & $1.747\pm0.065$ & $235.06\pm0.51$ & $0.00$ & M & M13 \\
MCPS-105 & 05:07:39.88 & -67:17:38.0 & $16.556\pm0.022$ & $1.759\pm0.033$ & $277.58\pm0.59$ & $0.00$ & M & M13 \\
MCPS-106 & 05:07:42.05 & -67:17:05.5 & $16.899\pm0.027$ & $1.682\pm0.037$ & $243.45\pm0.55$ & $0.00$ & M & M13 \\
MCPS-111 & 05:07:47.94 & -67:23:11.2 & $16.599\pm0.031$ & $2.012\pm0.084$ & $242.68\pm0.76$ & $0.00$ & M & M13 \\
MCPS-118 & 05:07:56.13 & -67:17:51.5 & $16.802\pm0.029$ & $1.600\pm0.038$ & $299.40\pm0.49$ & $0.00$ & M & M13 \\
MCPS-124 & 05:08:04.86 & -67:36:10.0 & $16.670\pm0.063$ & $1.517\pm0.075$ & $262.77\pm0.43$ & $0.00$ & M & M13 \\
MCPS-126 & 05:08:06.77 & -67:37:28.2 & $16.775\pm0.023$ & $1.923\pm0.045$ & $234.44\pm0.60$ & $0.00$ & M & M13 \\
MCPS-135 & 05:08:12.78 & -67:31:37.0 & $16.569\pm0.024$ & $1.596\pm0.049$ & $289.09\pm0.43$ & $0.00$ & M & M13 \\
MCPS-136 & 05:08:13.09 & -67:36:51.6 & $16.827\pm0.025$ & $1.533\pm0.047$ & $272.33\pm0.45$ & $0.00$ & M & M13 \\
MCPS-137 & 05:08:15.20 & -67:26:49.6 & $16.691\pm0.031$ & $1.788\pm0.051$ & $230.93\pm0.46$ & $0.00$ & M & M13 \\
MCPS-139 & 05:08:17.64 & -67:18:24.2 & $16.776\pm0.070$ & $1.819\pm0.074$ & $297.20\pm0.57$ & $0.00$ & M & M13 \\
MCPS-141 & 05:08:18.66 & -67:36:10.6 & $16.450\pm0.023$ & $1.823\pm0.044$ & $259.56\pm0.56$ & $0.00$ & M & M13 \\
MCPS-142 & 05:08:18.82 & -67:24:53.9 & $16.607\pm0.028$ & $1.596\pm0.048$ & $254.21\pm0.42$ & $0.00$ & M & M13 \\
MCPS-154 & 05:08:30.01 & -67:32:33.1 & $16.503\pm0.040$ & $1.968\pm0.056$ & $231.60\pm0.74$ & $0.00$ & M & M13 \\
MCPS-156 & 05:08:31.03 & -67:27:46.8 & $16.919\pm0.036$ & $1.573\pm0.054$ & $292.88\pm0.48$ & $0.00$ & M & M13 \\
MCPS-157 & 05:08:32.98 & -67:35:42.9 & $16.337\pm0.040$ & $1.803\pm0.055$ & $268.78\pm0.64$ & $0.00$ & M & M13 \\
MCPS-161 & 05:08:37.12 & -67:18:36.6 & $16.361\pm0.024$ & $1.900\pm0.033$ & $237.30\pm0.58$ & $0.00$ & M & M13 \\
MCPS-162 & 05:08:37.53 & -67:31:24.6 & $16.693\pm0.028$ & $1.805\pm0.052$ & $278.47\pm0.54$ & $0.00$ & M & M13 \\
MCPS-165 & 05:08:40.05 & -67:26:05.8 & $16.696\pm0.023$ & $1.632\pm0.045$ & $311.85\pm0.42$ & $0.00$ & M & M13 \\
MCPS-166 & 05:08:40.29 & -67:33:48.8 & $16.452\pm0.028$ & $1.924\pm0.048$ & $266.18\pm0.69$ & $0.00$ & M & M13 \\
MCPS-167 & 05:08:40.51 & -67:29:19.9 & $16.753\pm0.027$ & $1.623\pm0.048$ & $285.36\pm0.55$ & $0.00$ & M & M13 \\
MCPS-168 & 05:08:41.70 & -67:20:13.9 & $16.658\pm0.023$ & $2.008\pm0.034$ & $212.62\pm0.70$ & $0.00$ & M & M13 \\
MCPS-172 & 05:08:47.60 & -67:26:05.4 & $16.397\pm0.032$ & $1.563\pm0.053$ & $295.20\pm0.50$ & $0.00$ & M & M13 \\
MCPS-176 & 05:08:51.75 & -67:37:12.3 & $16.757\pm0.179$ & $1.695\pm0.184$ & $307.53\pm0.65$ & $0.00$ & M & M13 \\
MCPS-183 & 05:09:01.66 & -67:35:30.0 & $16.708\pm0.028$ & $1.999\pm0.051$ & $299.60\pm0.71$ & $0.00$ & M & M13 \\
MCPS-184 & 05:09:01.74 & -67:26:12.7 & $16.475\pm0.026$ & $1.828\pm0.047$ & $255.23\pm0.54$ & $0.00$ & M & M13 \\
MCPS-189 & 05:09:05.46 & -67:32:01.8 & $16.803\pm0.045$ & $1.554\pm0.060$ & $284.73\pm0.65$ & $0.00$ & M & M13 \\
MCPS-190 & 05:09:06.14 & -67:31:15.8 & $16.582\pm0.027$ & $1.617\pm0.055$ & $340.95\pm0.46$ & $0.00$ & M & M13 \\
MCPS-193 & 05:09:09.03 & -67:35:05.2 & $16.876\pm0.034$ & $1.589\pm0.052$ & $268.29\pm0.72$ & $0.00$ & M & M13 \\
MCPS-195 & 05:09:11.76 & -67:26:26.7 & $16.732\pm0.090$ & $1.577\pm0.099$ & $240.95\pm0.54$ & $0.00$ & M & M13 \\
MCPS-200 & 05:09:25.37 & -67:30:22.9 & $16.646\pm0.036$ & $1.485\pm0.054$ & $243.73\pm0.60$ & $0.00$ & M & M13 \\
\hline
\end{tabular}
\begin{tablenotes}
 \item $^{\rm a}$ {Photometric source that the target were selected from: H stands for \textit{HST} and M stands for MCPS.}
 \item $^{\rm b}$ {Spectroscopic source the LOS velocities were measured from: M2FS stands for this work, M13 stands for \citet{Mackey13}, and COMB stands for combined.}
\end{tablenotes}
\end{threeparttable}
\end{table*}

